Dynamic Grasping with a "Soft" Drone: From Theory to Practice

Rigid grippers used in existing aerial manipulators require precise positioning to achieve successful grasps and transmit large contact forces that may destabilize the drone. This limits the speed during grasping and prevents "dynamic grasping", where the drone attempts to grasp an object while moving. On the other hand, biological systems (e.g., birds) rely on compliant and soft parts to dampen contact forces and compensate for grasping inaccuracy, enabling impressive feats. This paper presents the first prototype of a soft drone -- a quadrotor where traditional (i.e., rigid) landing gears are replaced with a soft tendon-actuated gripper to enable aggressive grasping. We provide three key contributions. First, we describe our soft drone prototype, including electro-mechanical design, software infrastructure, and fabrication. Second, we review the set of algorithms we use for trajectory optimization and control of the drone and the soft gripper; the algorithms combine state-of-the-art techniques for quadrotor control (i.e., an adaptive geometric controller) with advanced soft robotics models (i.e., a quasi-static finite element model). Finally, we evaluate our soft drone in physics simulations (using SOFA and Unity) and in real tests in a motion-capture room. Our drone is able to dynamically grasp objects of unknown shape where baseline approaches fail. Our physical prototype ensures consistent performance, achieving 91.7% successful grasps across 23 trials. We showcase dynamic grasping results in the video attachment. Video Attachment: https://youtu.be/mqbj8mEyCdk

==> tex/aggressiveLanding.tex <==
%!TEX root = ../main.tex

\section{Aggressive Landing}
\label{sec:aggressiveLanding}
Whereas traditional quadrotors must decelerate to a safe velocity before landing in order to prevent component damage, the \red{soft drone's} inherent compliance dampens impact forces and enables safe landings at high velocities. This allows for the execution of aggressive trajectories where the time to execute a landing is short. 
%The configuration of the gripper upon landing can be optimized to minimize impact forces. We assume the quadrotor remains level upon impact with the ground, so that the attitude of the quadrotor can be neglected in the optimization. We restrict our motion to the vertical plane and assume no collision occurs in the lateral direction. Leveraging symmetry, there are four state variables to optimize: the front cable in the front facing pair of fingers $c_1$, the rear cable in the front facing pair of fingers $c_2$, and the front and rear cables in the rear facing pair of fingers $c_3$ and $c_4$. Upper and lower bounds $c_{max}$ and $c_{min}$, respectively, are placed on each cable to prevent extreme deformations of the fingers. In addition. the Young's Modulus, $E$, can be included in the optimization, if desired. The impact velocity, or the velocity of the quadrotor the instant the gripper makes contact with the ground, is denoted as $\vec{V}$. Let $t_x$ denote the collision time in the horizontal direction; the time it takes for the quadrotor to come to rest after touching the ground. Simililarly, $t_z$ denotes the collision time in the vertical direction. Let $m$ denote the total mass of the platform. The impact force of the collision can then be defined as:

The landing problem consists of finding the optimal gripper configuration to mitigate landing forces for a given state $X_c$, the quadrotor's state immediately before collision. We aim to find optimal values for the initial states $(\initialMY, \initialrestlengths)$. We treat the collision as time-invariant and hold the cable lengths $\initialrestlengths$ constant over the course of the collision. 

Collision dynamics of soft materials are difficult to analytically solve. \red{need citation} We adopt a data-driven approach and use a learned differentiable model to approximate the landing forces. We sample $\{((\initialMX, \initialMY, \initialrestlengths)^{(i)},  F^{(i)})\}_{i=1}^N$ data points in simulation and train a deep neural net in a supervised fashion. We define the force metric $F$ to penalize high impact forces during landing for a given quadrotor state $\initialMX$:

%Our model directly learns relations from cable lengths, $\initialrestlengths$, to an objective function $\landingobjective$ which penalizes high forces during landing for a given quadrotor state $\initialMX$:

\begin{equation}
\begin{array}{rcl}
\hspace{-2mm} 
    F  \label{eq:optLanding}
     = \hspace{-9mm}& \hspace{-2mm}
     \displaystyle  \int_{\collisiontime}^{\infty} f^2(\initialMX, \initialMY, \initialrestlengths, t) \dt
     \\
    
\end{array}
\end{equation}

where $\collisiontime$ denotes the instant the collision starts and $f$ denotes force. In practice, we evaluate this integral by replacing the upper bound with a constant, $\resttime$, such that the soft drone is approximately at rest.  

We use a gradient based approach to solve for the optimal gripper state. We formulate our optimal control problem as:

\begin{equation}
\begin{array}{rcl}
\hspace{-2mm} 
    (\initialMY^\star, \initialrestlengths^\star)  \label{eq:optLanding}
     = \hspace{-9mm}& \hspace{-2mm}
     \displaystyle  \argmin_{l} F(\initialMX, \initialMY, \initialrestlengths)
%     \\
%    & \hspace{-4mm}  \subject & 
%        \minrestlength \leq \restlength \leq \maxrestlength
\end{array}
\end{equation}
\red{worth mentioning that there are bounds on the cable legths and its projected gradient descent?}
We compute the network jacobian $\frac{d\mathbf{F}}{d\initialrestlengths}$ using analytical derivatives provided by Pytorch. We then use stochastic gradient descent to find the optimal cable lengths.



%\begin{equation}
%\begin{array}{rcl}
%\hspace{-2mm} 
%    \landingobjective  \label{eq:optLanding}
%     = \hspace{-9mm}& \hspace{-2mm}
%     \displaystyle  \sqrt{ \frac{1}{\collisiontime} \int_{\collisionstart}^{\collisionstart + \collisiontime} \landingforce^2(\initialMX, \initialMY, \initialrestlengths) \dt}
%     \\
%    
%\end{array}
%\end{equation}
%
%where the cost functional $\landingforce$ descrives the forces 
%
%
%In the above formulation we assume that propeller forces are zero during landing and that $\restlengths^\star$ has no dependence on time.
%
% 
% \begin{equation}
%\begin{array}{rcl}
%\hspace{-2mm} 
%    \vec{F}_{ave} = m\langle \frac{\vec{V}_x}{t_x(E, c_1,c_2,c_3,c_4)} , 0, \frac{\vec{V}_z}{t_z(E, c_1,c_2,c_3,c_4)} \rangle
%\end{array}
%\end{equation}
% 
% The desired Young's modulus and cable lengths can be formulated as an optimal control problem:
%\begin{equation}
%\begin{array}{rcl}
%\hspace{-2mm} 
%    (E^\star, c_1^\star, c_2^\star, c_3^\star, c_4^\star)  \label{eq:optControl}
%     = \hspace{-9mm}& \hspace{-2mm}
%     \displaystyle \argmin_{c_1, c_2, c_3, c_4} &
%     \norm{F_{ave}(m,\vec{V},E,c_1,c_2,c_3,c_4)}
%     \\
%    & \hspace{-4mm}  \subject & 
%        c_{min} \leq c_1, c_2, c_3, c_4 \leq c_{max}
%\end{array}
%\end{equation}
%\red{dont know best way to fix the test overflow in (5)}
%
%This problem is solved through gradient descent where the gradients $\frac{dF_{ave}}{dE}$ and $\frac{dF_{impact}}{dc_{i}}$ (for $i=1,2,3,4$) are computed numerically using simulation results.
%
%The optimization was ran at the upper bound of $\vec{V}$ to determine the optimal value of $E$ for landing, which evaluated to be \num{1e6} $N/m^2$. 




==> tex/extended_abstract.tex <==
%!TEX root = ../main.tex

We develop the first prototype of a \emph{\softDrone} -- a quadrotor combined with
an actuated soft robot and demonstrate its use in dynamic aerial grasping.

Rigid grippers used in existing aerial manipulators require precise positioning to 
achieve successful grasps and transmit large contact forces that may destabilize the drone.  This limits the speed during grasping and prevents ``dynamic grasping'', 
where the drone attempts to grasp an object while moving \cite{Thomas14bioinspiration}. 
On the other hand, biological systems (\eg birds) rely on compliant and soft parts to dampen contact forces and compensate for grasping inaccuracy, enabling impressive feats. Soft manipulators passively conform to the grasped object, enabling tolerance to imprecisions and reducing the need for explicit grasp analysis; this is an example of \emph{morphological computation}, the exploitation of passive mechanical elements to supplement explicit control. 
Compliance in aerial systems is a growing research area \cite{Cabellero18iros, Deng20arxiv, Ramon19iros}, with works specifically considering manipulation, but focusing on differentially flat
systems with limited degrees of freedom. By contrast, our paper utilizes techniques from the emerging discipline of \emph{soft robotics}~\cite{Bern19rss, Rus15nature} to plan for a system with nominally infinite degrees of freedom and which is no longer differentially flat.

In our \emph{\softDrone}, traditional (\ie~rigid) landing gears are replaced with a soft tendon-actuated gripper to enable aggressive grasping.
We provide three key contributions.
First, we describe our \softDrone prototype, including electro-mechanical design, software infrastructure, and fabrication: an \textit{Intel Aero Ready To Fly} quadrotor is retrofitted with a modular tendon-actuated silicone gripper modeled after a human hand and built around an \emph{Arduino Due} microcontroller. 

Second, we review the set of algorithms we use for trajectory optimization and control of the drone and the soft gripper. Our \softDrone is tasked with grasping an object of unknown shape, given the coordinates of its centroid. We implement a decoupled approach for control and planning, combining:
(i) an adaptive geometric controller and a minimum-snap trajectory optimization for the quadrotor (rigid) base, bringing the quadrotor to a feasible grasp pose, and 
(ii) a quasi-static finite element model and control-space interpolation for the soft gripper, defining a trajectory for the tendon lengths controlling the gripper which maximizes the chance of a successful grasp based on the nominal quadrotor trajectory.

Finally, we evaluate the effectiveness of our \softDrone in photo-realistic physics simulations (using SOFA and Unity) and in real tests. 
Our experiments show that
(i) in simulation, the adaptive controller converges regardless of the soft payload 
and ensures smaller errors compared to a standard geometric controller,
(ii) in simulation, our system reliably achieves aggressive grasps (at up to 2\SI{}{m/s}) of objects of unknown shape while a rigid manipulator fails,
(iii) in real tests, our soft drone ensures successful dynamic grasps (at up to 0.2\SI{}{m/s}) in 21 out of 23 consecutive tests, 
despite unmodeled aerodynamic effects.

We showcase these results in the video attachment {\small \url{https://www.youtube.com/watch?v=mqbj8mEyCdk}} and the preprint {\small \url{https://arxiv.org/pdf/2103.06465.pdf}}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\columnwidth]{new_slide_attempt}

    \caption{
    We develop the first prototype of a \emph{soft drone}, where 
  an actuated soft robot replaces the landing gear of a drone for dynamic grasping. 
    (a) Temporal sequence showing grasping at \SI{0.2}{m/s} in Unity-SOFA     physics simulator, 
    (b) Dynamic grasping in real tests. \label{fig:timelapse}}
\end{figure}


==> tex/relatedWork.tex <==
%!TEX root = ../main.tex

\section{Related Work}
\label{sec:relatedWork}

\red{Related work should focus a bit more aerial grasping systems}


\myParagraph{Compliant Aerial Manipulation}
Aerial manipulation with compliant, under-actuated and un-actuated components has been the subject of extensive research; however, this has been restricted to components with limited degrees of freedom and in which the combined system is differentially flat.
Cable-slung loads (F{\"o}hn\setal~\cite{Foehn17rss}, Sreenath\setal~\cite{Sreenath13icra}) are a well-studied under-actuated payload, but are differentially flat and 
%incapable of imposing 
are typically designed not to impose a torque on the aerial platform. The continuously deformable cable is either treated as massless or reduced to a finite number of links (Goodarzi\setal~\cite{Goodarzi14acc}). 
Thomas\setal~\cite{Thomas14bioinspiration} carry out aggressive aerial manipulation inspired by birds of prey using an under-actuated gripper, which can potentially grasp complex objects 
(see also Pounds\setal~\cite{Pounds11icra} and Backus\setal~\cite{Backus14iros}), but focus on the case of a suspended object which avoids unplanned collisions
% since unplanned collisions 
%  can cause instability 
 through the gripper. % and failures in the grasp. 
% Compliance in aerial grasp has been recognized as essential due to  
% precision limitations and platform instability, 
% and under-actuation enables grasp of arbitrary objects without explicit computation (Pounds\setal~\cite{Pounds11icra}, Backus\setal~\cite{Backus14iros}).  
The AEROARMS project (\cite{Cabellero18iros}, \cite{Ollero18ram}) explored the use of a manipulator with a flexible link to minimize disturbance on the aerial platform, but did not model or account for its impact on the drone dynamics.
% restrict the testing to cases where the compliance itself does not impact the dynamics.} 
Yuksel\setal~\cite{yuksel16iros} show differential flatness for aerial manipulators with arbitrary but finite numbers of  rigid or compliant joints; this result does not hold for the continuously deformable case. 
Kotaru\setal~\cite{Kotaru17acc} show that a standard geometric controller can stabilize a quadrotor and payload attached via an elastic cable (modeled as a spring with a single degree of freedom).
Ramon\setal~\cite{Ramon19iros} propose soft landing gear (similar in spirit to our design), but do not model the soft component nor its interaction with the quadrotor controller or control the soft landing gear beyond a binary open/close; moreover, the work focuses on landing rather than manipulation.

\myParagraph{Aggressive Landing}
\red{There exists substantial research on quadrotor landing on moving platforms (https://arxiv.org/pdf/1909.11071.pdf and related work). However, these works typically attempt to match the quadrotor speed to that of the platform; landing with a substantial relative velocity between quadrotor and platform appears relatively unstudied. Even in the case of a moving platform, landing often takes substantially upwards of 10 seconds; the maximum quadrotor speed for quick landing in extant work appears to be $1.2~\SI{}{m/s}$.}

	
\myParagraph{Morphing Drones}
\red{\textbf{Josh: do we need this section?}}
While not being targeted at manipulation, a recent set of papers investigates  the design of UAV platforms that can mechanically change shape to tolerate collisions or fit into narrow gaps.
{Mintchev\setal~\cite{Mintchev17ral} use insect-inspired structural compliance in a quadrotor frame to minimize impact damage, but this compliance does not affect the quadrotor dynamics during flight.} 
Falanga\setal~\cite{Falanga18ral} develop a drone that can fold its arms to fit into narrow gaps;
% in which the moment of inertia and center of mass position are potentially variable; 
morphological adaptability is limited to the plane so that the resulting dynamics can be expressed in closed form. 

Other related work includes quadrotors with tilting body or propellers 
(Ryll\setal~\cite{Ryll13icra-tiltingPropellers,Ryll15tro-tiltingPropellers}, Hintz\setal~\cite{Hintz14icuas-morphingDrone}, Riviere\setal~\cite{Riviere18softRobotics-morphingDrone}), 
scissor-like foldable quadrotors (Zhao\setal~\cite{Zhao17iros-deformableDrones}), 
 quadrotors with sprung-hinge-based foldable arms (Bucki and Mueller~\cite{Bucki19icra-morphingDrones}),
 and small-winged drones with morphing wing design (Di Luca\setal~\cite{DiLuca17interfaceFocus-morphingWings}). 
Contrarily to these works we consider a quadrotor carrying a soft gripper and prove that such a payload does not destroy the asymptotic stability of an existing geometric controller by 
Lee\setal~\cite{Lee10cdc-geometricControl}.


\myParagraph{Soft Robotics}
Continuously deformable, entirely compliant robots represent the extremum of the trend towards compliance and under-actuation.  However, traditional rigid-body modeling and control techniques fall short when confronted with infinite degrees of freedom. The emerging discipline of soft robotics has developed principled approaches to allow control of these systems, opening a new frontier in manipulation. 
Rus and Tolley~\cite{Rus15nature} and Thuruthel\setal~\cite{Thuruthel18softrobotics} provide a comprehensive review 
of soft robotics and soft manipulation.
% provide a comprehensive overview.
% We refer the readers to~\cite{Rus15nature, Thuruthel18softrobotics} for a comprehensive overview.
King\setal~\cite{King18humanoids}, Manti\setal~\cite{Manti15SoftRobotics}, and Hassan\setal~\cite{Hassan15embc} design bio-inspired tendon-actuated soft grippers. Marchese\setal~\cite{Marchese14icra,Marchese15icra} implement kinematics and trajectory optimization for hydraulic soft manipulators based on piecewise-constant-curvature approximations. Bern\setal~\cite{Bern17iros,Bern19rss} and Duriez\setal~\cite{Duriez13icra} model the kinematics and dynamics of tendon-actuated soft robots using finite element methods. 
These works have not been applied in the context of aerial manipulation, where the soft manipulator becomes a time-varying payload for the UAV and impacts its dynamics.

